The Llama 3 Herd of Models

Modern artificial intelligence (AI) systems are powered by foundation models. This paper presents a new set of foundation models, called Llama 3. It is a herd of language models that natively support multilinguality, coding, reasoning, and tool usage. Our largest model is a dense Transformer with 405B parameters and a context window of up to 128K tokens. This paper presents an extensive empirical evaluation of Llama 3. We find that Llama 3 delivers comparable quality to leading language models such as GPT-4 on a plethora of tasks. We publicly release Llama 3, including pre-trained and post-trained versions of the 405B parameter language model and our Llama Guard 3 model for input and output safety. The paper also presents the results of experiments in which we integrate image, video, and speech capabilities into Llama 3 via a compositional approach. We observe this approach performs competitively with the state-of-the-art on image, video, and speech recognition tasks. The resulting models are not yet being broadly released as they are still under development.

==> appendices/lc_safety/lc_safety_app.tex <==

\subsection{Long-context Safety Mitigation Details} \label{app:lc_safety_mitigation}

\textbf{Supervised finetuning datasets.}
To mitigate many-shot jailbreaking risks (MSJ), we train our long-context models to respond in a safe manner, even when presented with demonstrations of unsafe behavior in context. We construct SFT datasets comprising $k$-shot examples, formatted as multi-turn dialogues, as follows:: 1 example = [ $k$ demonstrations | target query | target response ].

We extract target queries and responses from adversarial and borderline SFT datasets, maintaining a 1:2 ratio between the two. We create demonstration pairs (<prompt, response>) by following the protocol of \cite{anil2024many}, with both benign/borderline (B) and harmful (H) content, resulting in the following combinations: BB, BH, HB, HH.

We create three types of MSJ mitigation datasets:
\begin{itemize}
    \item \textit{Mixed:} Each example includes a mix of BB, BH, HB, and HH demonstration pairs in equal proportions within the context.
    \item \textit{Repeated }(\cite{anil2024many}'s strategy): Each example contains only one type of pair, with an equal proportion of BB/BH/HB/HH-only examples across the dataset.
    \item \textit{Combined: } The dataset is evenly split between "mixed" and "repeated" examples.
\end{itemize}
We also vary the maximum number of shots:
\begin{itemize}
    \item \textit{1 to 16 shots}: The dataset includes 1, 2, 4, 8, and 16-shot examples in equal proportions.
    \item \textit{1 to 128 shots}: The dataset includes 1, 2, 4, 8, 16, 32, 64, and 128-shot examples in equal proportions.
\end{itemize}
The combination of dataset type (mixed/repeated/combined) and maximum number of shots (1 to 16 / 1 to 128) yields six datasets for experimentation. Our baseline is a version of Llama 3 8B finetuned on a data mix that already includes a limited amount of short-context safety data. We train six 8B models, each by adding one of the MSJ mitigation datasets to the baseline data mix.

\textbf{Results.} Our mitigation strategies show a strong balance between safety and helpfulness, as evidenced by the performance on both safety and helpfulness benchmarks.

\textbf{Robustness to many-shot jailbreaking.}
We evaluate the effectiveness of our mitigation strategies against many-shot jailbreaking (MSJ) risks using our internal benchmark. As shown in Fig. \ref{fig:msj_ablation_results}, the baseline model is vulnerable to MSJ, with a violation rate (VR) that increases up to 31\% as the number of shots increases up to 256. In contrast, models finetuned on MSJ mitigation data exhibit significantly reduced VR.
Specifically, we observe the following:
\begin{itemize}
    \item 1 to 16 shots: Models trained on 1 to 16 shots MSJ mitigation data achieve a VR of 5\% for 16-shot attacks, an approximately 70\% reduction in VR. For attacks with > 16 shots, we observe a gradual increase as the number of shots increases, but VR remains below 13\% even for 256-shot attacks. 
    \item 1 to 128 shots: The model trained on \textit{1 to 128 shots, mixed} MSJ mitigation data maintains a VR consistently below 10\% even for 256-shot attacks, demonstrating more effective mitigation.
\end{itemize}
Note that \cite{anil2024many} suggest that finetuning is sufficient for mitigating MSJ in long context models with bounded context length but not for arbitrary context lengths.
Interestingly, our results suggest that our strategy of mixing BB, BH, HB, and HH demonstration pairs within the context is more effective than simply repeating these patterns (as in \cite{anil2024many}), when increasing the number of shots for the attack. This suggests that the model may benefit from learning to recognize and adapt to context switching. Next, we provide new insights into the impact of this mitigation strategy for MSJ on other important aspects of model performance, including long-context (LC) helpfulness, short-context (SC) safety and SC helpfulness.

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{appendices/lc_safety/figs/llama3_msj_ablations.pdf}
    \caption{Effectiveness of supervised finetuning against many-shot jailbreaking attack.}
    \label{fig:msj_ablation_results}
\end{figure}

\textbf{Long-context helpfulness.}
As shown in Table \ref{table:msj-lc-helpfulness}, we observe no significant impact of training on MSJ mitigation data in InfiniteBench, and notably, no regression was detected in LongbookQA and LongbookChoice.

On ZeroScrolls, we observe a drop on QuALITY (multiple-choice questions over long articles and stories) in most of our ablation experiments, except for the \textit{1 to 128 shots, repeated }MSJ mitigation dataset. We observe no regression on other ZeroScrolls subtasks.


\begin{table}[]
\begin{tabular}{@{}lllllll@{}}
\toprule
                                & \multicolumn{3}{l}{ZeroScrolls} & \multicolumn{2}{l}{InfiniteBench} & NIH          \\
                                & QuALITY  & SQuALITY  & Qasper  & LongbookQA    & LongbookChoice    & Multi-needle \\ \midrule
8B Baseline                     & 0.714     & 0.237     & 0.335   & 0.213         & 0.629             & 0.98         \\
8B MSJ 1 to 16, mixed     & 0.476     & 0.245     & 0.358   & 0.29          & 0.686             & 0.978        \\
8B MSJ 1 to 128, mixed    & 0.571     & 0.245     & 0.381   & 0.259              & 0.651                  & 0.981        \\
8B MSJ 1 to 16, repeated  & 0.429     & 0.249     & 0.458   & 0.271         & 0.655             & 0.975        \\
8B MSJ 1 to 128, repeated & 0.762     & 0.241     & 0.35    & 0.249         & 0.607             & 0.975        \\
8B MSJ 1 to 16, combined  & 0.619     & 0.237     & 0.346   & 0.256         & 0.677             & 0.973        \\
8B MSJ 1 to 128, combined & 0.619     & 0.238     & 0.4     & 0.299         & 0.624             & 0.969        \\ \bottomrule
\end{tabular}
\caption{Impact of MSJ mitigation on long-context helpfulness performance. \label{table:msj-lc-helpfulness}}
\end{table}

\textbf{Short-context safety.}
Using our internal SC safety benchmarks, we find that after supervised finetuning on MSJ mitigation data, the SC violation rate is greatly reduced with only a minor increase to the false refusal rate (Table \ref{table:msj-sc-safety}).





\begin{table}
\centering

\begin{tabular}{| l | l | l |}
\hline
 & \textbf{Violation Rate} & \textbf{False Refusal Rate} \\
\hline
8B Baseline  & 29.59\% & 1.91\% \\

8B MSJ 1 to 16 shots, mixed  & 12.79\% & 2.02\% \\

8B MSJ 1 to 128 shots, mixed & 13.24\% & 2.37\% \\

8B MSJ 1 to 16 shots, repeated  & 12.60\% & 2.16\% \\

8B MSJ 1 to 128 shots, repeated  & 13.52\% & 2.51\% \\

8B MSJ 1 to 16 shots, combined  & 14.61\% & 2.44\% \\

8B MSJ 1 to 128 shots, combined  & 14.06\% & 2.37\% \\
\hline

\end{tabular}
\caption{Impact of MSJ mitigation on short-context safety metrics. \label{table:msj-sc-safety}}
\end{table}



\textbf{Short-context helpfulness.}
We also evaluate the impact of our MSJ mitigation strategies on SC helpfulness using several public and internal benchmarks. Our results in Table \ref{table:msj-sc-helpfulness} show no degradation on academic benchmarks, including MMLU, except for a $\approx1.7\%$decrease on the MATH benchmark. Overall, mitigating MSJ via supervised finetuning does not significantly impact SC helpfulness performance.


\begin{table}[]
\begin{tabular}{@{}lllllll@{}}
\toprule
                                      & MMLU   & ARC-Challenge & GPQA   & HumanEval & GSM8K  & MATH   \\ \midrule
8B baseline & 69.2\% & 85.0\%        & 29.0\% & 64.0\%    & 81.9\% & 40.6\% \\
MSJ 1 to 16 shots, mixed              & 69.5\% & 84.8\%        & 28.6\% & 62.8\%    & 83.2\% & 38.9\% \\
MSJ 1 to 128 shots, mixed             & 69.3\% & 84.5\%        & 28.1\% & 64.6\%    & 82.2\% & 38.9\% \\
MSJ 1 to 16 shots, repeated           & 69.2\% & 84.6\%        & 29.2\% & 63.4\%    & 82.5\% & 39.4\% \\
MSJ 1 to 128 shots, repeated          & 69.2\% & 84.5\%        & 30.1\% & 61.6\%    & 81.8\% & 38.6\% \\
MSJ 1 to 16 shots, combined           & 69.1\% & 85.4\%        & 28.3\% & 64.0\%    & 82.4\% & 39.2\% \\
MSJ 1 to 128 shots, combined          & 69.0\% & 84.5\%        & 30.1\% & 64.6\%    & 82.9\% & 38.5\% \\ \bottomrule
\end{tabular}
\caption{Impact of MSJ mitigation on short-context helpfulness performance. \label{table:msj-sc-helpfulness}}
\end{table}


==> appendices/pretraining_results.tex <==
\section{Pretrained model evaluation}

\subsection{Per-benchmark results}\label{appendix:full_results_pretraining}

\begin{table}
\centering
\input{results/tables/reading_comprehension_benchmarks}
\caption{Non-aggregated pretraining evaluation results for the Knowledge and Reasoning categories.}
\label{table:full_results_pretraining_reading_comprehension}
\end{table}

\begin{table}
\centering
\input{results/tables/knowledge_benchmarks}
\caption{Non-aggregated pretraining evaluation results for the Knowledge and Reasoning categories.}
\label{table:full_results_pretraining_knowledge}
\end{table}

\begin{table}
\centering
\input{results/tables/commonsense_benchmarks}
\caption{Non-aggregated pretraining evaluation results for the Commonsense reasoning and understanding benchmarks.}
\label{table:full_results_pretraining_commonsense}
\end{table}

\begin{table}
\centering
\input{results/tables/math_reasoning_benchmarks}
\caption{Non-aggregated pretraining evaluation results for math and reasoning benchmarks.}
\label{table:full_results_math_reasoning}
\end{table}

\begin{table}
\centering
\input{results/tables/code_benchmarks}
    \caption{Non-aggregated pretraining evaluation results for long context (\TBD{still missing}) and code.}
\label{table:full_results_code}
\end{table}

\begin{table}
\centering
    \input{results/tables/general_benchmarks}
    \caption{Non-aggregated pretraining evaluation results for aggregate benchmarks.}
\label{table:full_results_general}
\end{table}


\section{Reproducibility: Prompts and fewshots examples}\label{appendix:prompt_details}

\begin{table}[]
\small
\centering
\setlength{\tabcolsep}{1.5pt}
\begin{tabular}{lcccc}
\toprule
\small
\bfseries Benchmark & \bfseries License & \bfseries \# samples & \bfseries \# few-shot & \bfseries Metric \\
\midrule
\makecell[l]{Adv SQuAD \citep{jia-liang-2017-adversarial}} & &  & 1 &  F1 \\
\midrule
\makecell[l]{AGIEval \citep{zhong2023agieval}} & MIT & 2546 & 3-5 & Accuracy \\
\midrule
\makecell[l]{ARC-C \citep{clark2018think}} & Apache 2.0 & 1165 & 0 & Accuracy \\
\midrule
\makecell[l]{Big Bench Hard \citep{suzgun-etal-2023-challenging}} & Apache 2.0 &  6511 & 3 (CoT) & EM (micro avg) \\
\midrule
\makecell[l]{CommonSenseQA \\\citep{talmor-etal-2019-commonsenseqa}} & & 1140 & 7 & Accuracy \\
\midrule
\makecell[l]{DROP \citep{dua-etal-2019-drop}} &  & 9536  & 3 & F1\\
\midrule
\makecell[l]{Dynabench SQuAD \citep{}} & &  &  &  \\
\midrule
\makecell[l]{GSM8k \citep{cobbe2021training}} & MIT & 1319 & 8 & EM maj1@1 \\
\midrule
\makecell[l]{GSM-Plus \\ \citep{cobbe2021training}} & &  & 8  & EM maj1@1 \\
\midrule
\makecell[l]{HumanEval \citep{chen2021evaluating}} & MIT & 164 & 0 & Pass@1 \\
\midrule
\makecell[l]{InfinityBench \citep{zhang2024infty}} & &  & & F1 \\
\midrule
\makecell[l]{L-Eval \citep{an2023eval}} & &  & & \\
\midrule
\makecell[l]{MATH \citep{hendrycks2021measuring}} & MIT & 5000 & 4 & EM maj1@1 \\
\midrule
\makecell[l]{MBPP \citep{austin2021program}} & & 500 & 3 & Pass@1 \\
\midrule
\makecell[l]{MMLU \citep{hendrycks2021mmlu}} & MIT & 14042 & 5 & Accuracy (micro) \\
\midrule
    \makecell[l]{MMLU-Pro \citep{wang2024mmlu}} &  & 12032 & 5 & Accuracy (micro) \\
\midrule
\makecell[l]{Needle in Haystack\\ \citep{kuratov2024search}} & &  & & \\
\midrule
\makecell[l]{OpenBookQA\\ \citep{mihaylov-etal-2018-suit}} & &  & 0 & Accuracy \\
\midrule
\makecell[l]{PAWS \citep{}} & &  & 5  &  Accuracy \\
\midrule
\makecell[l]{PiQA \citep{bisk2020piqa}} & Academic Free & 1838 & 0 & Accuracy \\
\midrule
\makecell[l]{RACE \citep{lai-etal-2017-race}} & &  & 0 & Accuracy (micro)  \\
\midrule
\makecell[l]{QuAC \citep{choi-etal-2018-quac}} & &  & 1 & F1 \\
\midrule
\makecell[l]{QQP \citep{quoraFirstQuora}} & &  5 &  Accuracy &  \\
\midrule
\makecell[l]{SCROLLS \citep{shaham-etal-2022-scrolls}} & &  & & \\
\midrule
\makecell[l]{SiQA \cite{sap-etal-2019-social}} &   & 1954 & 0 & Acc \\
\midrule
\makecell[l]{SQuAD v2 \citep{rajpurkar-etal-2018-know}} & &  & 5 & EM \\
\midrule
    \makecell[l]{SQuAD (for adversarial plots)\\ \citep{rajpurkar-etal-2018-know}} & &  & 1 & EM \\
\midrule
\makecell[l]{TriviaQA \cite{joshi-etal-2017-triviaqa}} & Apache 2.0 & 11313 & 5 & EM \\
\midrule
\makecell[l]{TruthfulQA \citep{lin-etal-2022-truthfulqa}} & & & 0 & MC2\_score \\
\midrule
\makecell[l]{Winogrande \citep{sakaguchi2021winogrande}} & & &  5 & Accuracy \\
\midrule
\makecell[l]{WorldSense \\\citep{benchekroun2023worldsense}} &  & 87048 & 0 & Accuracy (macro)\\
\bottomrule
\end{tabular}
\caption{Few-shot and metric settings for all pretraining benchmarks used in the paper, in alphabetical order.}\label{table:pretraining_benchmark_details}
\end{table}

\subsection{Paraphrases for MMLU prompt robustness experiment}

In Table~\ref{table:mmlu_paraphrase_variations}, we report the paraphrases we use for our prompt robustness experiments with MMLU in Section~\ref{subsec:robustness}.
Each instruction is followed by five few-shot examples, followed by the word \texttt{Answer:};
We compute scores by comparing the log probabilities of all possible answer labels.

\begin{table}
    \begin{tabular}{ll}
        \toprule
        \textit{Default} & \makecell[l]{The following are multiple choice questions (with answers) about \{\{ subject \}\}}. \\
        \midrule
        \textit{Variation 1} & \makecell[l]{The following are multiple choice questions (with answers) about \{\{ subject \}\}. Choose\\ the best answer for the final question.} \\

        \midrule
        \textit{Variation 2} & \makecell[l]{Given the following questions and four candidate answers (A, B, C and D), choose the\\ best answer for the final question.} \\
        \midrule
        \textit{Variation 3} & \makecell[l]{You are an expert in solving MCQ questions covering vast knowledge. Analyse the \\following questions (with answers) and select the correct answer for the final question.} \\
        \midrule
        \textit{Variation 4} & \makecell[l]{You are an expert in solving questions on \{\{ subject \}\}. Analyse the following questions\\ (with answers) and choose the best answer for the final question.} \\
        \midrule
        \textit{Variation 5} & \makecell[l]{Solve the following multiple choice questions on \{\{ subject \}\}.}\\
    \bottomrule
    \end{tabular}
    \caption{Paraphrased instructions used for prompt robustness experiments described in Section~\ref{subsec:robustness}. Each instruction is followed by five few-shot examples, followed by `\texttt{Answer: }'.}\label{table:mmlu_paraphrase_variations}
\end{table}

\subsection{Contamination analysis}\label{app:contamination_analysis}

In Figure \ref{figure:contamination_analysis}, we show how both the percent of data marked contaminated and the estimated performance gain changes with the ratio of tokens occurring in an 8-gram also present in the training corpus. 
For some datasets, such as for instance SiQA and HellaSwag, there is a clear right threshold, and the estimated performance gain changes stably with the threshold.
For other datasets, the behaviour is much more erratic, with large spikes or negative performance gains, suggesting that the chosen contamination method may be suboptimal for those specific datasets.
A dataset for which this is easy to spot is WorldSense, where the found contamination comprises of false positives consisting of templated phrases such as \emph{`The Taj Mahal and the Sagrada Familia'}, that are part of but not relevant to the asked question.
Note that when close to 100\% of a dataset is marked contaminated, the reported estimations will be particularly unreliable, because the sample of `clean' samples is too small to get a reliable estimate.

\begin{figure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/agi_english}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/bbh}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/boolq}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/csqa}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/drop}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/gsm8k}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/hellaswag}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/human_eval}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/math}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/mbpp}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/mmlu}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/mmlu_pro}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/nq}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/obqa}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/piqa}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/siqa}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/squad}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/winogrande}
    \end{subfigure}
    \begin{subfigure}[b]{0.246\textwidth}
    \includegraphics[width=\textwidth]{assets/pretraining_results/contamination_analysis/worldsense}
    \end{subfigure}
    \caption{Estimation of performance gain and estimated contamination per threshold.}\label{figure:contamination_analysis}
\end{figure}


==> posttraining/assets/chat_format.tex <==

\begin{table}[ht]
  \centering
  \begin{tabular}{ll>{\raggedright}p{8cm}l}
    \toprule
    Index & Header & Message Content & Termination \\
    \midrule
    0 & system & Environment: ipython \linebreak Tools: brave\_search \linebreak Cutting Knowledg Date: December 2023 \linebreak Today Date: 23 Jul 2024 & <eot\_id> \\
    \midrule
    1 & user & What's the temperature in Seattle today? & <eot\_id> \\
    \midrule
    2 & assistant &  <|python\_tag|> brave\_search.call(query="Seattle temperature today") & <eom\_id> \\
    \midrule
    3 & ipython & \{"query": "Seattle temperature today", "top\_k": [search results omitted]\} & <eom\_id> \\
    \midrule
    4 & assistant & The current temperature in Seattle is 69.8°F (21°C). & <eot\_id> \\
    \bottomrule
  \end{tabular}
  \caption{\llamathree chat dialogue format for tool-use and code execution.}
  \label{tab:chat_format}
\end{table}


==> posttraining/assets/code_difficulty_prompt.tex <==
\begin{figure}
  
\footnotesize
\begin{framed}

You are the coding expert and your task is to evaluate the difficulty of a given coding prompt. \\

Here is the definition of three difficulty level (easy, medium, hard) for coding prompts: \\

\#\# Easy

The prompt is undergraduate level questions or leetcode easy question. The prompt requires limited domain /algorithmics knowledge or implementation context (architecture, libraries, pre-existing code). There is little ambiguity in the prompt (in case of underspecification, good default behaviors are easy to come up with or not important), limited complexity of specifications (in number of instructions). The solution of prompt is easy to explain (e..g, code doesn’t need comments to be understood) and to test for/debug (e.g., limited corner cases). \\

For example:

\begin{itemize}
    \item Implement the factorial function in <language X>.
    \item How to count the number of lines in a file called log.txt in bash?
    \item How can I parse a json file in <language X/library Y>?
    \item What’s the complexity of getting the n-th element from a list in Python?
\end{itemize} 

\vspace{5mm}

\#\# Medium 

The prompt is masters level questions or leetcode medium question. The prompt requires knowledge of standard algorithms and data structures to get an optimal solution, knowledge of common libraries and concepts. May require additional code context. There is Medium ambiguity in the prompt (e.g., needs to come up with reasonable ad-hoc data representation or class structure without explicit guidance), multiple requirements should be satisfied or multiple bugs should be found. \\

For example:

\begin{itemize}
    \item Compute the average value in the column .metrics.accuracy for elements with .compile=True in the file metrics.jsonl in bash
    \item Compute the longest increasing subsequence in a list. Implement the solution in <language X>. 
    \item How can I use the twitter python API to send a tweet automatically?
\end{itemize}

\vspace{5mm}
\#\# Hard

The prompt is domain expert level or leetcode hard question. The prompt requires understanding of complex and long code/log snippet). The prompt requires expert domain knowledge, or information on the specific application or deployment scenario, including substantial specific API/code context. Finding good solutions of the prompt needs non-trivial design decisions regarding data structures, algorithms or code architecture/design patterns. Finding a solution requires solving several non-trivial subproblems or finding non-trivial bugs. Problem involves tricky corner cases, explaining the solution to a non-expert requires adding context. \\

For example:

\begin{itemize}
    \item Example 1 (leetcode hard type):
For my homework I need to write a python function that implements regular expression matching, with support for '.' and '+', where '.' stands for any character and '+' matches 1 or more of the preceding element. The function has signature match(s, p) where s is the input string and p the regexp pattern. The matching may be partial. I can't use any regexp library for this assignment. Could you help with that?
\item Example 2 (expert knowledge):
What would be AdagradW, the equivalent of AdamW for Adagrad? Implement AdagradW in Python.

\item Example 3: (objective-oriented design question) Make a pong game in <language X>

\item Example 4 (complex plot):
I have a pandas dataframe with the columns "decoding", "Capabilities", "Fine-tuning", "Model size", "HE pass@1", "MBPP pass@1". I want a seaborn figure with two scatterplots side-by-side. The two plots show "HE pass@1" vs "MBPP pass@1", using different subsets of the data: The first plot uses the data with "decoding" equal to 0.1, the second plot uses
"greedy" for "decoding".

\item Example 5 (documentation/comments/unit tests/commits for complex and long code/log snippet)

\item Example 6 (create example usages/code Summarization of complex and long code snippet):
\end{itemize}

Based on the definition of the three difficulty levels, please evaluate the difficulty of the last user prompt. You need to provide your explanation first. Then, output the level of difficulty **strictly following this XML format**: <difficulty></difficulty>. For example, <difficulty>Easy</difficulty>

\end{framed}

  \caption{\textbf{Llama code difficulty scoring prompt}: We use the above prompt to score the difficulty of synthetically generated coding data.}
  \label{fig:llama_difficulty_coding_prompt}
\end{figure}





==> posttraining/assets/code_quality_filter.tex <==
\begin{figure}
  

\begin{framed}

You are a code reviewer for the following question answer pairs. Your job is to rate the quality of each answer based on the following criteria: \\

\begin{itemize}
\item \textbf{Bug Identification} (1 point): \\
    - Check if you can find any bug in the code. Provide a reasoning chain of why the answer is or is not buggy and the final result. \\

\item \textbf{User Intention} (1 point): \\
    - Check if the answer satisfy the user's need or not. Provide a reasoning chain about what's the final answer of the model and why it satisfy the user's intent or not. \\
    
\end{itemize} 

I will now present you with a coding-related question-answer exchange between an AI system and a user. \\

Analyze the Question: Consider the AI's responses in the context of the user's queries. Apply each criterion to evaluate how well the AI's responses meet these standards. \\

Justify Your Scoring: For each point awarded, provide a brief explanation (up to 50 words per criterion) justifying why the AI's responses meet the specific criterion. \\
        
Final Score: Conclude your evaluation with the total score out of 2, formatted as Final Score: <SCORE>/2. This should be the sum of the points awarded for each criterion. \\

Note: Be sure to be careful and strict, even one small bug can cause the failure of the program. Ensure that the final score does not exceed 2 points. Do not award partial points.

\end{framed}

  \caption{\textbf{Llama code quality filter prompt}: We use the above prompt to score synthetically generated coding data.}
  \label{fig:llama_quality_coding_prompt}
\end{figure}





==> posttraining/assets/helpfulness_difficulty_prompt.tex <==
\begin{figure}

\small
\begin{framed}

Our task is to evaluate the difficulty of a given user prompt. \\
Here is the definition of three difficulty levels (Easy, Medium, Hard) for user prompts:\\


\#\# Easy

Prompt is a single ask/requirement/constraint for the model presented as a single statement OR prompt is a single statement without ask/requirement/constraints.
Prompt would not require subject matter expertise to understand. \\

Examples:
\begin{itemize}
\item Illustrate and explain the proper use of a semi-colon.
\item How do I uninvite my brother to my wedding?
\item I've been having trouble sticking to my healthy diet lately. Give me some motivational words or tips to help me make better food choices and achieve my health goals.
\end{itemize}

\vspace{5mm}

\#\# Medium

Prompt includes 2-4 asks/requirements/constraints for the model AND would not require subject matter expertise to produce a response. \\

Examples:
\begin{itemize}
\item My neighbors blast loud music all night, and I can’t sleep. I’ve tried talking to them directly, as well as calling 311 but nothing has changed. What else do you think I can try?
\item How do I ask my boss for a raise? I think I’m underpaid but my boss never has time for me.
\item Pretend you’re Bugs Bunny. I’m Elmer Fudd. How would you greet me?
\item Write me a funny haiku about dogs.
\end{itemize}

\vspace{5mm}

\#\# Hard

Prompt contains 5 or more asks/requirements/constraints for the model OR requires subject matter expertise above and beyond “common knowledge” in order to respond. \\

Examples:
\begin{itemize}
\item Write a poem to say sorry to my dog because I didn't spend enough time with it. The poem should have 26 lines where each line begins with Z, Y, X, ..., A, respectively, and always ends with h. The poem cannot contain any animal words.
\item Sort the following words alphabetically, and in the result remove the first and the fourth words while capitalize the rest: sioux fortescue purloin percept helmsman friend friends. Append a new lower-case word that is an animal living in Antarctica. Output the result with numbered bullets.
\item Handling long-sequence inputs presents a significant challenge to the KV-cache of Transformers.  Can we address this challenge better by training Transformers with more GPUs?
\end{itemize}

Based on the definition of the three difficulty levels, please evaluate the difficulty of the last user prompt. You need to provide your explanation first. Then, output the level of difficulty strictly following this XML format: <difficulty></difficulty>. For example, <difficulty>Easy</difficulty>

\end{framed}

\caption{\textbf{Llama English difficulty scoring prompt}: We use the above prompt to score the difficulty of general English data.}
\label{fig:llama_difficulty_helpful_prompt}
\end{figure}


==> posttraining/assets/instag_prompt.tex <==
\begin{figure}
  
\begin{framed}

You are a tagging system that provides useful tags for instruction intentions to distinguish instructions for a helpful AI assistant.
Below is an interaction between a user and an AI assistant. \\

Please provide coarse-grained tags, such as ``Spelling and Grammar Check'' and ``Cosplay'', to identify main intentions of above interaction. 

Your answer should be a list including titles of tags and a brief explanation of each tag.
Your response have to strictly follow this JSON format: [\{``tag'': str, ``explanation'': str\}].\\

\emph{Example of Dialog}: <EXAMPLE> \\
\emph{Tags}: <EXAMPLE> \\
\emph{Reason}: <EXAMPLE> 

\end{framed}

  \caption{\textbf{Llama instag prompt}: We use the above prompt to perform intention tagging for general English data. We supply demonstrations to the model using a set of human-tagged results.}
  \label{fig:instag_prompt}
\end{figure}





==> posttraining/assets/quality_filter.tex <==














\begin{figure}
  

\begin{framed}

I would like to rate conversations with an AI assistant using the following rubric: \\

\begin{itemize}
\item \textbf{Accuracy} (1 point): \\
    - The AI should not make mistakes anywhere in the conversation.\\
    - The AI responses should be free of factual or reasoning errors or self-contradictions. All mathematical calculations must be accurate.\\
    - Analyze the responses carefully for factually incorrect claims. Do not award points for false or dubious information, stereotypes or generalizations, or fabricated events or people. \\

    \emph{Example of Inaccurate Dialog}: <EXAMPLE> \\
    \emph{Reason}: <EXAMPLE> \\

\item \textbf{Instruction Following} (1 point): \\
    - The AI responses should address all parts of the user's query and accurately follows its instructions. \\
    - The AI should not unnecessarily resort to ethical guidelines when the user's query is obviously harmless. \\

    \emph{Example of Poorly Followed Instructions}: <EXAMPLE> \\
    \emph{Reason}: <EXAMPLE> \\

\item \textbf{Tone and Presentation} (1 point): \\
    - The AI responses should be to-the-point, clear, and free of spelling and grammatical mistakes. \\
    - The AI responses should have a tone and style that makes sense given the user's query.\\
    - The AI responses should be formatted clearly and easy-to-read.\\
    - The AI responses should not be unnecessarily verbose, repetitive, unclear, second-guessing, judgemental, or preachy.\\

    \emph{Example of Poor Tone and Presentation}: <EXAMPLE>\\
    \emph{Reason}: <EXAMPLE>
\end{itemize} 

Now I will provide you an conversation between an AI system and a user. \\

Please rate the quality of the AI responses using the above rubric. \\

First, provide a brief justification of your score. \\

Then, conclude with your rating in the format FINAL SCORE: <SCORE>/3. \\

Be extremely strict and objective; only award the point if the criterion is fully satisfied. \\

If any part of the criterion is not satisfied, however minor, do not award the point. Do not award partial points.

\end{framed}

  \caption{\textbf{Llama quality filter prompt}: We use the above prompt to score synthetically generated helpfulness data. We supply demonstrations to the model using a validation set of human-verified quality assessments of synthetic dialogues.}
  \label{fig:llama_quality_prompt}
\end{figure}





==> results/tables/code_benchmarks.tex <==
\begin{NiceTabular}{lccc}
	\CodeBefore
	\Body
	\toprule
	& \multicolumn{2}{c}{\textbf{Code}} \\
	\midrule
	& HumanEval & MBPP & \textit{Winrate}\\
\cmidrule{2-3}
	Llama 3 8B & \textbf{37.2 \scriptsize{$\pm$7.4}}& \textbf{47.6 \scriptsize{$\pm$4.4}} & \textit{2}\\
	Llama 2 7B &12.8 \scriptsize{$\pm$5.1}& 22.0 \scriptsize{$\pm$3.6} & \textit{0}\\
	Llama 2 13B &18.9 \scriptsize{$\pm$6.0}& 27.6 \scriptsize{$\pm$3.9} & \textit{0}\\
	Mistral 7B &\textbf{30.5 \scriptsize{$\pm$7.0}}& \textbf{47.5 \scriptsize{$\pm$4.4}} & \textit{2}\\
	Gemma 7B &\textbf{32.3 \scriptsize{$\pm$7.2}}& \textbf{44.4 \scriptsize{$\pm$4.4}} & \textit{2}\\
	\cmidrule{2-3}
	Llama 3 70B & \textbf{58.5 \scriptsize{$\pm$7.5}}& 66.2 \scriptsize{$\pm$4.1} & \textit{1}\\
	Mixtral 8x22B &45.1 \scriptsize{$\pm$7.6}& \textbf{71.2 \scriptsize{$\pm$4.0}} & \textit{1}\\
	Qwen2 72B &\textbf{64.6 \scriptsize{$\pm$7.3}}& \textbf{76.9 \scriptsize{$\pm$3.7}} & \textit{2}\\
	Llama 2 70B &29.3 \scriptsize{$\pm$7.0}& 45.2 \scriptsize{$\pm$4.4} & \textit{0}\\
	\cmidrule{2-3}
	Llama 3 405B & 61.0 \scriptsize{$\pm$7.5}& \textbf{73.4 \scriptsize{$\pm$3.9}} & \textit{1}\\
	GPT4 &67.0 \scriptsize{$\pm$7.2}& - & \textit{0}\\
	Nemotron &57.3 \scriptsize{$\pm$7.6}& - & \textit{0}\\
	Gemini Ultra &\textbf{74.4 \scriptsize{$\pm$4.2}}& - & \textit{1}\\
	\bottomrule
\end{NiceTabular}


==> results/tables/commonsense_benchmarks.tex <==
\begin{NiceTabular}{lcccccc}
	\CodeBefore
	\Body
	\toprule
	& \multicolumn{5}{c}{\textbf{Commonsense}} \\
	\midrule
	& CommonSenseQA & PiQA & SiQA & OpenBookQA & WinoGrande & \textit{Winrate}\\
\cmidrule{2-6}
	Llama 3 8B & \textbf{75.0 \scriptsize{$\pm$2.5}}& \textbf{81.0 \scriptsize{$\pm$1.8}}& \textbf{49.5 \scriptsize{$\pm$2.2}}& \textbf{45.0 \scriptsize{$\pm$4.4}}& \textbf{75.7 \scriptsize{$\pm$2.0}} & \textit{5}\\
	Llama 2 7B &57.9 \scriptsize{$\pm$2.9}& 78.9 \scriptsize{$\pm$1.9}& \textbf{48.4 \scriptsize{$\pm$2.2}}& \textbf{44.4 \scriptsize{$\pm$4.4}}& 73.0 \scriptsize{$\pm$2.1} & \textit{2}\\
	Llama 2 13B &67.4 \scriptsize{$\pm$2.7}& \textbf{80.4 \scriptsize{$\pm$1.8}}& \textbf{50.6 \scriptsize{$\pm$2.2}}& \textbf{44.8 \scriptsize{$\pm$4.4}}& \textbf{75.9 \scriptsize{$\pm$2.0}} & \textit{4}\\
	Mistral 7B &\textbf{71.2 \scriptsize{$\pm$2.6}}& \textbf{83.0 \scriptsize{$\pm$1.7}}& \textbf{48.2 \scriptsize{$\pm$2.2}}& \textbf{47.8 \scriptsize{$\pm$4.4}}& \textbf{78.1 \scriptsize{$\pm$1.9}} & \textit{5}\\
	Gemma 7B &\textbf{74.4 \scriptsize{$\pm$2.5}}& \textbf{81.5 \scriptsize{$\pm$1.8}}& \textbf{51.8 \scriptsize{$\pm$2.2}}& \textbf{52.8 \scriptsize{$\pm$4.4}}& \textbf{74.7 \scriptsize{$\pm$2.0}} & \textit{5}\\
	\cmidrule{2-6}
	Llama 3 70B & 84.1 \scriptsize{$\pm$2.1}& \textbf{83.8 \scriptsize{$\pm$1.7}}& 52.2 \scriptsize{$\pm$2.2}& \textbf{47.6 \scriptsize{$\pm$4.4}}& \textbf{83.5 \scriptsize{$\pm$1.7}} & \textit{3}\\
	Mixtral 8x22B &82.4 \scriptsize{$\pm$2.2}& \textbf{85.5 \scriptsize{$\pm$1.6}}& 51.6 \scriptsize{$\pm$2.2}& \textbf{50.8 \scriptsize{$\pm$4.4}}& \textbf{84.7 \scriptsize{$\pm$1.7}} & \textit{3}\\
	Qwen2 72B &\textbf{90.5 \scriptsize{$\pm$1.7}}& \textbf{83.6 \scriptsize{$\pm$1.7}}& \textbf{62.5 \scriptsize{$\pm$2.1}}& \textbf{49.0 \scriptsize{$\pm$4.4}}& \textbf{85.1 \scriptsize{$\pm$1.7}} & \textit{5}\\
	Llama 2 70B &78.9 \scriptsize{$\pm$2.4}& \textbf{82.5 \scriptsize{$\pm$1.7}}& 50.8 \scriptsize{$\pm$2.2}& \textbf{49.2 \scriptsize{$\pm$4.4}}& \textbf{82.2 \scriptsize{$\pm$1.8}} & \textit{3}\\
	\cmidrule{2-6}
	Llama 3 405B & \textbf{85.8 \scriptsize{$\pm$2.0}}& \textbf{85.6 \scriptsize{$\pm$1.6}}& \textbf{53.7 \scriptsize{$\pm$2.2}}& \textbf{49.2 \scriptsize{$\pm$4.4}}& 82.2 \scriptsize{$\pm$1.8} & \textit{4}\\
	GPT4 &-& -& -& -& \textbf{87.5 \scriptsize{$\pm$1.5}} & \textit{1}\\
	Nemotron &-& -& -& -& \textbf{89.5 \scriptsize{$\pm$1.4}} & \textit{1}\\
	Gemini Ultra &-& -& -& -& - & \textit{0}\\
	\bottomrule
\end{NiceTabular}


==> results/tables/fact_score_post.tex <==
\begin{NiceTabular}{lcc}
	\CodeBefore
	\Body
	\toprule
&FActScore & \textit{Winrate}\\
\cmidrule{2-2}
	Llama 3 8B & \textbf{62.1 \scriptsize{$\pm$4.3}} & \textit{1}\\
	Gemma 9B - it &\textbf{67.9 \scriptsize{$\pm$4.1}} & \textit{1}\\
	Mistral 7B Instruct &48.7 \scriptsize{$\pm$4.4} & \textit{0}\\
	\midrule
	Llama 3 70B & \textbf{74.1 \scriptsize{$\pm$3.8}} & \textit{1}\\
	Mixtral-8x22B Instruct &\textbf{69.9 \scriptsize{$\pm$4.0}} & \textit{1}\\
	GPT-3.5 Turbo &\textbf{76.1 \scriptsize{$\pm$3.7}} & \textit{1}\\
	\midrule
	Llama 3 405B & 77.0 \scriptsize{$\pm$3.7} & \textit{0}\\
	GPT-4 (0125) &\textbf{87.9 \scriptsize{$\pm$2.9}} & \textit{1}\\
	GPT-4 Omni &\textbf{88.3 \scriptsize{$\pm$2.8}} & \textit{1}\\
	Claude-3.5 Sonnet &80.0 \scriptsize{$\pm$3.5} & \textit{0}\\
	Nemotron &70.1 \scriptsize{$\pm$4.0} & \textit{0}\\
	\bottomrule
\end{NiceTabular}


==> results/tables/general_benchmarks.tex <==
\begin{NiceTabular}{lccccc}
	\CodeBefore
	\Body
	\toprule
	& \multicolumn{4}{c}{\textbf{General}} \\
	\midrule
	& MMLU & MMLU-Pro & AGIEval & BIG-Bench Hard & \textit{Winrate}\\
\cmidrule{2-5}
	Llama 3 8B & \textbf{65.6 \scriptsize{$\pm$0.8}}& \textbf{35.6 \scriptsize{$\pm$0.9}}& \textbf{47.8 \scriptsize{$\pm$1.9}}& \textbf{64.2 \scriptsize{$\pm$1.2}} & \textit{4}\\
	Llama 2 7B &45.7 \scriptsize{$\pm$0.8}& 18.9 \scriptsize{$\pm$0.7}& 29.1 \scriptsize{$\pm$1.8}& 39.0 \scriptsize{$\pm$1.2} & \textit{0}\\
	Llama 2 13B &55.4 \scriptsize{$\pm$0.8}& 23.8 \scriptsize{$\pm$0.8}& 38.6 \scriptsize{$\pm$1.9}& 46.9 \scriptsize{$\pm$1.2} & \textit{0}\\
	Mistral 7B &62.5 \scriptsize{$\pm$0.8}& 30.7 \scriptsize{$\pm$0.8}& 42.7 \scriptsize{$\pm$1.9}& 56.8 \scriptsize{$\pm$1.2} & \textit{0}\\
	Gemma 7B &\textbf{64.3 \scriptsize{$\pm$0.8}}& 33.6 \scriptsize{$\pm$0.8}& \textbf{46.0 \scriptsize{$\pm$1.9}}& 57.7 \scriptsize{$\pm$1.2} & \textit{2}\\
	\cmidrule{2-5}
	Llama 3 70B & 79.0 \scriptsize{$\pm$0.7}& 52.0 \scriptsize{$\pm$0.9}& 64.6 \scriptsize{$\pm$1.9}& \textbf{81.6 \scriptsize{$\pm$0.9}} & \textit{1}\\
	Mixtral 8x22B &77.8 \scriptsize{$\pm$0.7}& 49.9 \scriptsize{$\pm$0.9}& 61.5 \scriptsize{$\pm$1.9}& 79.5 \scriptsize{$\pm$1.0} & \textit{0}\\
	Qwen2 72B &\textbf{84.3 \scriptsize{$\pm$0.6}}& \textbf{55.8 \scriptsize{$\pm$0.9}}& \textbf{72.4 \scriptsize{$\pm$1.7}}& \textbf{82.4 \scriptsize{$\pm$0.9}} & \textit{4}\\
	Llama 2 70B &69.1 \scriptsize{$\pm$0.8}& 37.0 \scriptsize{$\pm$0.9}& 53.6 \scriptsize{$\pm$1.9}& 65.7 \scriptsize{$\pm$1.2} & \textit{0}\\
	\cmidrule{2-5}
	Llama 3 405B & \textbf{85.4 \scriptsize{$\pm$0.6}}& \textbf{59.6 \scriptsize{$\pm$0.9}}& \textbf{71.6 \scriptsize{$\pm$1.8}}& \textbf{85.9 \scriptsize{$\pm$0.8}} & \textit{4}\\
	GPT4 &\textbf{86.4 \scriptsize{$\pm$0.6}}& -& -& - & \textit{1}\\
	Nemotron &81.1 \scriptsize{$\pm$0.6}& -& -& \textbf{85.4 \scriptsize{$\pm$0.9}} & \textit{1}\\
	Gemini Ultra &83.7 \scriptsize{$\pm$0.6}& -& -& 83.6 \scriptsize{$\pm$0.9} & \textit{0}\\
	\bottomrule
\end{NiceTabular}


==> results/tables/knowledge_benchmarks.tex <==
\begin{NiceTabular}{lccc}
	\CodeBefore
	\Body
	\toprule
	& \multicolumn{2}{c}{\textbf{Knowledge}} \\
	\midrule
	& TriviaQA & TruthfulQA & \textit{Winrate}\\
\cmidrule{2-3}
	Llama 3 8B & 77.6 \scriptsize{$\pm$0.8}& \textbf{44.1 \scriptsize{$\pm$3.4}} & \textit{1}\\
	Llama 2 7B &72.1 \scriptsize{$\pm$0.8}& \textbf{38.7 \scriptsize{$\pm$3.3}} & \textit{1}\\
	Llama 2 13B &\textbf{79.6 \scriptsize{$\pm$0.7}}& 37.3 \scriptsize{$\pm$3.3} & \textit{1}\\
	Mistral 7B &76.6 \scriptsize{$\pm$0.8}& \textbf{41.7 \scriptsize{$\pm$3.4}} & \textit{1}\\
	Gemma 7B &72.6 \scriptsize{$\pm$0.8}& \textbf{45.1 \scriptsize{$\pm$3.4}} & \textit{1}\\
	\cmidrule{2-3}
	Llama 3 70B & \textbf{89.8 \scriptsize{$\pm$0.6}}& \textbf{51.0 \scriptsize{$\pm$3.4}} & \textit{2}\\
	Mixtral 8x22B &\textbf{88.8 \scriptsize{$\pm$0.6}}& \textbf{51.1 \scriptsize{$\pm$3.4}} & \textit{2}\\
	Qwen2 72B &85.6 \scriptsize{$\pm$0.6}& \textbf{54.8 \scriptsize{$\pm$3.4}} & \textit{1}\\
	Llama 2 70B &87.7 \scriptsize{$\pm$0.6}& 44.9 \scriptsize{$\pm$3.4} & \textit{0}\\
	\cmidrule{2-3}
	Llama 3 405B & \textbf{91.8 \scriptsize{$\pm$0.5}}& \textbf{49.7 \scriptsize{$\pm$3.4}} & \textit{2}\\
	GPT4 &-& - & \textit{0}\\
	Nemotron &-& - & \textit{0}\\
	Gemini Ultra &-& - & \textit{0}\\
	\bottomrule
\end{NiceTabular}


==> results/tables/math_reasoning_benchmarks.tex <==
\begin{NiceTabular}{lcccccc}
	\CodeBefore
	\Body
	\toprule
	& \multicolumn{5}{c}{\textbf{Math and Reasoning}} \\
	\midrule
	& GSM8K & MATH & ARC-C & DROP & WorldSense & \textit{Winrate}\\
\cmidrule{2-6}
	Llama 3 8B & \textbf{57.2 \scriptsize{$\pm$2.7}}& 20.3 \scriptsize{$\pm$1.1}& \textbf{79.7 \scriptsize{$\pm$2.3}}& \textbf{59.5 \scriptsize{$\pm$1.0}}& \textbf{45.5 \scriptsize{$\pm$0.3}} & \textit{4}\\
	Llama 2 7B &14.9 \scriptsize{$\pm$1.9}& 3.0 \scriptsize{$\pm$0.5}& 54.6 \scriptsize{$\pm$2.9}& 40.5 \scriptsize{$\pm$1.0}& 44.4 \scriptsize{$\pm$0.3} & \textit{0}\\
	Llama 2 13B &29.3 \scriptsize{$\pm$2.5}& 5.2 \scriptsize{$\pm$0.6}& 67.0 \scriptsize{$\pm$2.7}& 49.7 \scriptsize{$\pm$1.0}& 44.5 \scriptsize{$\pm$0.3} & \textit{0}\\
	Mistral 7B &\textbf{52.5 \scriptsize{$\pm$2.7}}& 13.1 \scriptsize{$\pm$0.9}& \textbf{78.2 \scriptsize{$\pm$2.4}}& 53.0 \scriptsize{$\pm$1.0}& 44.9 \scriptsize{$\pm$0.3} & \textit{2}\\
	Gemma 7B &46.4 \scriptsize{$\pm$2.7}& \textbf{24.3 \scriptsize{$\pm$1.2}}& \textbf{78.6 \scriptsize{$\pm$2.4}}& 56.3 \scriptsize{$\pm$1.0}& \textbf{46.0 \scriptsize{$\pm$0.3}} & \textit{3}\\
	\cmidrule{2-6}
	Llama 3 70B & 83.7 \scriptsize{$\pm$2.0}& 41.4 \scriptsize{$\pm$1.4}& \textbf{92.9 \scriptsize{$\pm$1.5}}& \textbf{79.6 \scriptsize{$\pm$0.8}}& 61.1 \scriptsize{$\pm$0.3} & \textit{2}\\
	Mixtral 8x22B &\textbf{88.4 \scriptsize{$\pm$1.7}}& 41.8 \scriptsize{$\pm$1.4}& 91.9 \scriptsize{$\pm$1.6}& 77.5 \scriptsize{$\pm$0.8}& 51.5 \scriptsize{$\pm$0.3} & \textit{1}\\
	Qwen2 72B &\textbf{89.5 \scriptsize{$\pm$1.7}}& \textbf{55.9 \scriptsize{$\pm$1.4}}& \textbf{95.0 \scriptsize{$\pm$1.2}}& 76.9 \scriptsize{$\pm$0.8}& \textbf{68.2 \scriptsize{$\pm$0.3}} & \textit{4}\\
	Llama 2 70B &57.9 \scriptsize{$\pm$2.7}& 13.6 \scriptsize{$\pm$1.0}& 85.4 \scriptsize{$\pm$2.0}& 70.1 \scriptsize{$\pm$0.9}& 45.5 \scriptsize{$\pm$0.3} & \textit{0}\\
	\cmidrule{2-6}
	Llama 3 405B & \textbf{89.0 \scriptsize{$\pm$1.7}}& \textbf{53.8 \scriptsize{$\pm$1.4}}& \textbf{96.1 \scriptsize{$\pm$1.1}}& \textbf{84.8 \scriptsize{$\pm$0.7}}& \textbf{63.7 \scriptsize{$\pm$0.3}} & \textit{5}\\
	GPT4 &\textbf{92.0 \scriptsize{$\pm$1.5}}& -& \textbf{96.3 \scriptsize{$\pm$1.1}}& 80.9 \scriptsize{$\pm$0.8}& - & \textit{2}\\
	Nemotron &-& -& \textbf{94.3 \scriptsize{$\pm$1.3}}& -& - & \textit{1}\\
	Gemini Ultra &\textbf{88.9 \scriptsize{$\pm$1.7}}& \textbf{53.2 \scriptsize{$\pm$1.4}}& -& 82.4 \scriptsize{$\pm$0.8}& - & \textit{2}\\
	\bottomrule
\end{NiceTabular}


==> results/tables/posttraining_metric_details.tex <==
\begin{table}
    \center
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{lrrl}
        \toprule
        \textbf{Benchmark} & \textbf{\# samples} & \textbf{\# few-shot} & \textbf{Metric} \\
        \midrule
        API-Bank~\citep{li2023api} & 391 & 0 & accuracy \\
        API-Bench~\citep{patil2023gorilla} & 1775 & 0 & accuracy \\
        ARC Challenge \citep{clark2018think} & 1165 & 0 & accuracy  \\
        BFCL~\citep{berkeley-function-calling-leaderboard} & 1700 & 0 & accuracy \\
        FActScore \citep{min2023factscore} & 500 & 0 & precision \\
        GPQA \citep{rein2023gpqagraduatelevelgoogleproofqa} & 448 & 0 & accuracy  \\
        GSM8K \citep{cobbe2021training} & 1319 & 8 & exact match  \\
        HumanEval \citep{chen2021evaluating} & 164 & 0 & pass@1  \\
        HumanEval+~\citep{liu2024your} & 164 & 0 & pass@1 \\
        IFEval \citep{zhou2023instruction} & 541 & 0 & prompt/instruction accuracy  \\
        InfiniteBench/En.QA \citep{zhang2024infty} & 351 & 0 & f1  \\
        InfiniteBench/En.MC \citep{zhang2024infty} & 229 & 0 & accuracy  \\
        MATH \citep{hendrycks2021measuring} & 5000 & 0/4 & sympy + judge  \\
        MBPP \citep{austin2021program} & 500 & 3 & pass@1 \\
        MBPP EvalPlus (base) \citep{liu2024your} & 378 & 0 & pass@1 \\
        MGSM \citep{shi2022languagemodelsmultilingualchainofthought} & 2750 & 8 & exact match  \\
        MMLU \citep{hendrycks2021mmlu} & 14042 & 0/5 & macro/micro accuracy  \\
        MMLU-Pro \citep{wang2024mmlu} & 12032 & 5 & macro/micro accuracy  \\
        MultiPL-E HumanEval ~\citep{cassano2022multiple} & 3025 & 0 & pass@1 \\
        MultiPL-E MBPP ~\citep{cassano2022multiple} & 7384 & 0 & pass@1  \\
        Needle-in-a-Haystack \citep{niah} & 225 & 0 & exact match  \\
        Nexus~\citep{srinivasan2023nexusraven} & 542 & 0 & accuracy \\
        ZeroSCROLLS/QuALITY \citep{zeroscrolls} & 21 & 0 & exact match  \\
        ZeroSCROLLS/Qasper \citep{zeroscrolls} & 28 & 0 & f1  \\
        ZeroSCROLLS/SQuALITY \citep{zeroscrolls} & 80 & 0 & rougeL  \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Few shot and metric settings for all posttraining benchmarks} used in the paper, in alphabetical order.
        \label{tab:posttraining_benchmark_metric_details}
    }
\end{table}


==> results/tables/reading_comprehension_benchmarks.tex <==
\begin{NiceTabular}{lcccc}
	\CodeBefore
	\Body
	\toprule
	& \multicolumn{3}{c}{\textbf{Reading Comprehension}} \\
	\midrule
	& SQuAD & QuAC & RACE & \textit{Winrate}\\
\cmidrule{2-4}
	Llama 3 8B & 77.0 \scriptsize{$\pm$0.8}& \textbf{44.9 \scriptsize{$\pm$1.1}}& \textbf{54.3 \scriptsize{$\pm$1.4}} & \textit{2}\\
	Llama 2 7B &72.3 \scriptsize{$\pm$0.8}& 39.5 \scriptsize{$\pm$1.1}& 51.1 \scriptsize{$\pm$1.4} & \textit{0}\\
	Llama 2 13B &72.2 \scriptsize{$\pm$0.8}& \textbf{44.9 \scriptsize{$\pm$1.1}}& \textbf{53.9 \scriptsize{$\pm$1.4}} & \textit{2}\\
	Mistral 7B &73.2 \scriptsize{$\pm$0.8}& \textbf{44.7 \scriptsize{$\pm$1.1}}& \textbf{53.0 \scriptsize{$\pm$1.4}} & \textit{2}\\
	Gemma 7B &\textbf{81.8 \scriptsize{$\pm$0.7}}& 42.4 \scriptsize{$\pm$1.1}& 48.8 \scriptsize{$\pm$1.4} & \textit{1}\\
	\cmidrule{2-4}
	Llama 3 70B & 81.8 \scriptsize{$\pm$0.7}& \textbf{51.1 \scriptsize{$\pm$1.1}}& \textbf{59.0 \scriptsize{$\pm$1.4}} & \textit{2}\\
	Mixtral 8x22B &\textbf{84.1 \scriptsize{$\pm$0.7}}& 44.9 \scriptsize{$\pm$1.1}& \textbf{59.2 \scriptsize{$\pm$1.4}} & \textit{2}\\
	Qwen2 72B &73.2 \scriptsize{$\pm$0.8}& \textbf{51.1 \scriptsize{$\pm$1.1}}& \textbf{60.8 \scriptsize{$\pm$1.4}} & \textit{2}\\
	Llama 2 70B &82.6 \scriptsize{$\pm$0.7}& \textbf{49.5 \scriptsize{$\pm$1.1}}& 56.2 \scriptsize{$\pm$1.4} & \textit{1}\\
	\cmidrule{2-4}
	Llama 3 405B & \textbf{81.8 \scriptsize{$\pm$0.7}}& \textbf{53.6 \scriptsize{$\pm$1.1}}& \textbf{58.1 \scriptsize{$\pm$1.4}} & \textit{3}\\
	GPT4 &-& -& - & \textit{0}\\
	Nemotron &-& -& - & \textit{0}\\
	Gemini Ultra &-& -& - & \textit{0}\\
	\bottomrule
\end{NiceTabular}


==> results/tables/speech_cvst2_ast_noagg.tex <==
\begin{NiceTabular}{lcccc}
	\CodeBefore
	\Body
	\toprule
	X$\rightarrow$English & Llama 3 8B & Llama 3 70B & Whisper v2 & SeamlessM4T v2 \\
	\midrule
	Portuguese	&	48.4	&	55.1	&	51.6	&	53.8	\\
	Indonesian	&	47.9	&	51.1	&	48.1	&	52.4	\\
	Arabic	&	45.5	&	48.6	&	39.7	&	46.7	\\
	Russian	&	43.9	&	50.3	&	43.3	&	53.6	\\
	Dutch	&	42.3	&	45.5	&	41.2	&	42.8	\\
	French	&	40.6	&	43.5	&	36.4	&	42.1	\\
	Spanish	&	40.2	&	43.8	&	40.1	&	42.9	\\
	German	&	38.0	&	42.0	&	36.3	&	39.9	\\
	Italian	&	37.3	&	41.1	&	30.9	&	40.0	\\
	Swedish	&	36.0	&	44.8	&	42.9	&	43.5	\\
	Turkish	&	28.8	&	31.8	&	28.3	&	33.1	\\
	Persian	&	24.7	&	26.6	&	19.3	&	27.2	\\
	Japanese	&	24.5	&	28.3	&	26.1	&	23.8	\\
	Chinese	&	15.2	&	23.8	&	18.0	&	22.2	\\
	Tamil	&	2.2	&	6.0	&	4.2	&	4.6	\\
	\midrule
	Average & 34.4& 38.8 & 33.8 & 37.9 \\
	\bottomrule
\end{NiceTabular}


==> results/tables/speech_fleurs_asr_noagg.tex <==
\begin{NiceTabular}{lcccc}
	\CodeBefore
	\Body
	\toprule
	Language &  Llama 3 8B & Llama 3 70B & Whisper v3 & SeamlessM4T v2 \\
	\midrule
	Italian	&	3.7	&	3.3	&	3.0	&	6.1	\\
	Spanish	&	3.8	&	3.1	&	2.8	&	6.6	\\
	Korean	&	4.8	&	3.7	&	3.1	&	7.2	\\
	English	&	5.7	&	4.5	&	4.1	&	7.4	\\
	Portuguese	&	5.7	&	4.5	&	4.1	&	9.2	\\
	Indonesian	&	5.8	&	5.0	&	6.1	&	9.5	\\
	French	&	6.3	&	5.6	&	5.3	&	8.4	\\
	German	&	6.5	&	5.7	&	4.9	&	8.2	\\
	Japanese	&	7.2	&	7.2	&	4.9	&	12.1	\\
	Hindi	&	7.8	&	6.1	&	17.0	&	11.0	\\
	Kannada	&	7.9	&	7.2	&	33.0	&	14.4	\\
	Russian	&	7.9	&	6.9	&	5.0	&	10.3	\\
	Dutch	&	7.9	&	6.6	&	5.2	&	9.7	\\
	Polish	&	8.4	&	6.6	&	4.6	&	10.2	\\
	Bengali	&	8.7	&	7.6	&	50.0	&	8.6	\\
	Vietnamese	&	8.8	&	7.4	&	8.6	&	9.9	\\
	Malayalam	&	8.9	&	7.9	&	--	&	12.8	\\
	Thai	&	9.0	&	7.7	&	8.4	&	11.3	\\
	Chinese	&	9.1	&	7.8	&	7.7	&	11.4	\\
	Gujarati	&	9.8	&	9.2	&	47.4	&	13.4	\\
	Marathi	&	10.1	&	8.3	&	34.1	&	13.9	\\
	Turkish	&	10.4	&	8.3	&	6.7	&	12.3	\\
	Tamil	&	10.7	&	10.5	&	18.3	&	15.0	\\
	Finnish	&	10.9	&	8.3	&	7.7	&	14.0	\\
	Romanian	&	11.3	&	8.4	&	8.2	&	11.0	\\
	Swedish	&	12.0	&	9.6	&	7.6	&	12.8	\\
	Czech	&	12.5	&	9.8	&	10.1	&	11.9	\\
	Persian	&	12.6	&	12.7	&	29.4	&	23.5	\\
	Swahili	&	12.8	&	12.7	&	34.1	&	15.0	\\
	Telugu	&	13.2	&	12.3	&	39.3	&	15.9	\\
	Greek	&	13.8	&	11.9	&	10.9	&	11.2	\\
	Arabic	&	14.0	&	13.0	&	9.6	&	14.8	\\
	Hungarian	&	18.6	&	11.8	&	12.9	&	13.9	\\
	Urdu	&	19.0	&	17.2	&	20.6	&	17.5	\\
	\midrule
	Average &9.6 & 8.2 &	14.4	&	11.8	 \\
	\bottomrule
\end{NiceTabular}


==> results/tables/speech_fleurs_ast_noagg.tex <==
\begin{NiceTabular}{lcccc}
	\CodeBefore
	\Body
	\toprule
	X$\rightarrow$English & Llama 3 8B & Llama 3 70B & Whisper v2 & SeamlessM4T v2 \\
	\midrule
	Portuguese	&	44.4	&	48.4	&	38.1	&	38.4	\\
	German	&	40.2	&	42.7	&	34.6	&	37.0	\\
	French	&	40.0	&	42.2	&	32.2	&	34.0	\\
	Swedish	&	37.6	&	43.2	&	35.3	&	36.9	\\
	Romanian	&	36.9	&	41.0	&	31.5	&	35.0	\\
	Indonesian	&	36.6	&	42.9	&	29.1	&	32.7	\\
	Arabic	&	36.0	&	40.9	&	25.5	&	34.6	\\
	Russian	&	33.0	&	36.9	&	27.8	&	30.2	\\
	Czech	&	32.9	&	37.4	&	27.8	&	34.0	\\
	Italian	&	31.9	&	34.6	&	23.6	&	26.5	\\
	Spanish	&	31.8	&	34.4	&	23.3	&	25.5	\\
	Swahili	&	31.4	&	37.9	&	7.2	&	31.1	\\
	Dutch	&	31.0	&	32.1	&	24.0	&	27.8	\\
	Persian	&	30.5	&	34.8	&	19.6	&	30.3	\\
	Finnish	&	29.6	&	34.5	&	22.1	&	28.0	\\
	Greek	&	28.7	&	31.6	&	23.7	&	27.1	\\
	Hindi	&	28.4	&	35.0	&	22.0	&	28.2	\\
	Turkish	&	28.3	&	36.9	&	26.6	&	30.7	\\
	Gujarati	&	27.8	&	33.3	&	16.2	&	31.4	\\
	Polish	&	26.4	&	29.1	&	22.3	&	24.4	\\
	Hungarian	&	26.3	&	32.3	&	21.2	&	27.8	\\
	Bengali	&	26.1	&	30.2	&	13.2	&	26.3	\\
	Malayalam	&	25.4	&	29.7	&	16.7	&	26.0	\\
	Urdu	&	25.3	&	30.0	&	17.2	&	24.4	\\
	Vietnamese	&	24.7	&	27.6	&	20.4	&	26.0	\\
	Kannada	&	24.7	&	28.8	&	11.6	&	25.1	\\
	Thai	&	23.7	&	26.9	&	16.1	&	23.2	\\
	Marathi	&	23.5	&	29.5	&	12.9	&	27.4	\\
	Telugu	&	23.5	&	25.0	&	12.5	&	25.1	\\
	Chinese	&	23.4	&	25.7	&	18.4	&	23.0	\\
	Korean	&	21.7	&	25.9	&	21.3	&	24.1	\\
	Japanese	&	21.0	&	25.3	&	18.9	&	18.2	\\
	Tamil	&	20.9	&	24.7	&	9.2	&	22.2	\\
	\midrule
	Average & 29.5 & 33.7 & 21.9 & 28.6 \\
	\bottomrule
\end{NiceTabular}

